Nonparametric identification is not enough, but randomized controlled trials are

We argue that randomized controlled trials (RCTs) are special even among settings where average treatment effects are identified by a nonparametric unconfoundedness assumption. This claim follows from two results of Robins and Ritov (1997): (1) with at least one continuous covariate control, no estimator of the average treatment effect exists which is uniformly consistent without further assumptions, (2) knowledge of the propensity score yields a uniformly consistent estimator and honest confidence intervals that shrink at parametric rates with increasing sample size, regardless of how complicated the propensity score function is. We emphasize the latter point, and note that successfully-conducted RCTs provide knowledge of the propensity score to the researcher. We discuss modern developments in covariate adjustment for RCTs, noting that statistical models and machine learning methods can be used to improve efficiency while preserving finite sample unbiasedness. We conclude that statistical inference has the potential to be fundamentally more difficult in observational settings than it is in RCTs, even when all confounders are measured.

==> xwtjpfhppcxfqdxsdjcpxzfggcqhvbdm/extra_figures.tex <==
\section{Additional Figures}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.39\textwidth]{figures/new_rmse_experiment1.pdf}
    \includegraphics[width=0.39\textwidth]{figures/new_rmse_experiment2.pdf}
    \includegraphics[width=0.39\textwidth]{figures/new_rmse_experiment3.pdf}
    \caption{The RMSE of the estimators which use the true propensity score when estimating the average treatment effect for a range of $n$ in the experimental setups outlined in Section \ref{sim_setups}}
    \label{fig:rmse_zoomed}
\end{figure}

\begin{figure}[H]
\centering
    \includegraphics[width=0.45\textwidth]{figures/rmse_table.pdf}
    \caption{The RMSE of all estimators which use the true propensity score when estimating the average treatment effect for a range of $n$ in the experimental setups outlined in Section \ref{sim_setups}}
    \label{fig:rmse_table}
\end{figure}


==> xwtjpfhppcxfqdxsdjcpxzfggcqhvbdm/proofs.tex <==
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{ex}[thm]{Example}

\makeatletter
\renewenvironment{proof}[1][\proofname] {\par\pushQED{\qed}\normalfont\topsep6\p@\@plus6\p@\relax\trivlist\item[\hskip\labelsep\bfseries#1\@addpunct{:}]\ignorespaces}{\popQED\endtrivlist\@endpefalse}
\makeatother


\definecolor{direct}{HTML}{FF0000}
\definecolor{indirect}{HTML}{FF9999}
\definecolor{dirin}{HTML}{990000}
\definecolor{control}{HTML}{999999}
\definecolor{directE}{HTML}{ED1C24}
\definecolor{indirectE}{HTML}{F69679}
\definecolor{controlE}{HTML}{999999}

\def\E{{\rm E}}
\def\V{{\rm V}}
\def\Cov{{\rm Cov}}
\def\I{{\rm I}}
\def\Supp{{\rm Supp}}
\def\Pr{P}
\def\Supphat{\text{S}\widehat{\text{up}}\text{p}}

\def\S{{\sigma}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\dd}{\mathbf{d}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\F}{\mathbf{F}}
\renewcommand{\S}{\mathbf{S}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\g}{\mathbf{g}}
\renewcommand{\r}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\tt}{\mathbf{t}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\LL}{\mathcal{L}}

\newcommand{\BBeta}{\boldsymbol{\beta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Alpha}{\boldsymbol{\alpha}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\arrowp}{\stackrel{p}{\rightarrow}}
\newcommand{\arrowd}{\stackrel{d}{\rightarrow}}
\newcommand{\arrowas}{\stackrel{a.s.}{\rightarrow}}
\newcommand{\approxsim}{\stackrel{approx.}{\sim}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\nn}{\nonumber}
\def\S{{\sigma}}
\renewcommand{\qed}{\space $\square$}

% Commands for inline arrowp and arrowd to avoid spacing problem
\makeatletter
\newcommand{\oset}[3][0ex]{
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-2\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother
\newcommand{\inlinearrowp}{\oset{p}{\rightarrow}}
\newcommand{\inlinearrowd}{\oset{d}{\rightarrow}}

% Commands for proper size and spacing of |
\newcommand{\bigvert}{\, \big | \,}
\newcommand{\Bigvert}{\, \Big | \,}
\newcommand{\biggvert}{\, \bigg | \,}
\newcommand{\Biggvert}{\, \Bigg | \,}

% No extra spacing with \left and \right
\delimitershortfall-1sp
%\mleftright

% Command for list intertext
\makeatletter
\newcommand{\listintertext}{\@ifstar\listintertext@\listintertext@@}
\newcommand{\listintertext@}[1]{
  \hspace*{-\@totalleftmargin}#1}
\newcommand{\listintertext@@}[1]{
  \hspace{-\leftmargin}#1}
\makeatother

%\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
%\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\allowdisplaybreaks[1]

\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}

\addtolength{\oddsidemargin}{-.25in}
	\addtolength{\evensidemargin}{-.25in}
	\addtolength{\textwidth}{.5in}
\addtolength{\textheight}{.2in}
\addtolength{\topmargin}{-.1in}

\makeatletter
\renewcommand*{\ext@figure}{lot}
\let\c@figure\c@table
\let\ftype@figure\ftype@table
\let\listoftableandfigures\listoftables
\renewcommand*\listtablename{Tables and Figures}
\makeatother



% Below added so that figures and table are numbered by subsection
%\usepackage{chngcntr}
%\counterwithin{figure}{subsection}
%\counterwithin{table}{subsection}
% threepartable added for table notes in applications of ch. 4
\makeatletter
\newcommand{\setword}[2]{
  \phantomsection
  #1\def\@currentlabel{\unexpanded{#1}}\label{#2}
}
\makeatother


\section{Proof of Proposition 4(a)}
Suppose that we have an RCT where SUTVA holds. Then $\hat \mu_{1,R}$ is finite-sample unbiased for $\mu_{1}$.

\begin{proof}

Much of the proof follows the exposition of \citet{aronowmiller}, Theorem 6.2.6.

%\begin{align*}
%   \E[ \hat \mu_{1,R}] & = \E\left[\frac{(Y_i -  g(W_i, \hat \beta_i))X_i}{\pi_i(W_i)} + n^{-1}\sum_{i=1}^n g(W_i, \hat \beta_i)\right] \\
%   & =  \E\left[\frac{Y_i X_i}{\pi_i(W_i)}\right] -  \E \left[\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)}\right] + \E n^{-1}\sum_{i=1}^n \left[g(W_i, \hat \beta_i)\right] \\
%      & =  \E\left[\E[\frac{Y_i X_i}{\pi_i(W_i)|W_i]}\right] -  \E \left[\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)}\right] + \E n^{-1}\sum_{i=1}^n \left[g(W_i, \hat \beta_i)\right] \\
%
%\end{align*}



Begin by decomposing into three terms:
\begin{align}
 \E[ \hat \mu_{1,R}] & = \E\left[n^{-1} \sum_{i=1}^n \left\{ \frac{(Y_i -  g(W_i, \hat \beta_i))X_i}{\pi_i(W_i)} + \sum_{i=1}^n g(W_i, \hat \beta_i) \right\}\right] \\
 & = \E\left[\frac{Y_i X_i}{\pi_i(W_i)}\right] -  \E \left[\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)}\right] + \E \left[g(W_i, \hat \beta_i)\right],
\end{align}
By linearity of expectations and unbiasedness of the sample mean.

We begin by examining the first term ($\E\left[\frac{Y_i X_i}{\pi_i(W_i)}\right]$), and first derive the analogous conditional expectation with respect to $W_i$. By definition,
\begin{align}
    \E\left[\frac{Y_i X_i}{\pi(W_i)} | W_i \right] =\E\left[Y_i \cdot \frac{X_i}{\Pr \left( X_i = 1 \vert W_i\right)} | W_i \right]
\end{align}
And by the potential outcomes model, 
\begin{align*}
    \E\bigg[Y_i \cdot\frac{X_i}{\Pr(X_i = 1 \vert W_i)} \biggvert W_i \bigg] = \E\bigg[Y_i(1) \cdot \frac{X_i}{\Pr \left(X_i = 1 \vert W_i\right)} \biggvert W_i \bigg].
\end{align*}
Then since ignorability holds, $Y_i(1) \independent X_i \vert W_i$, so:
\begin{align*}
\E\bigg[Y_i(1) \cdot \frac{X_i}{\Pr \left([X_i = 1 \vert W_i\right)} \biggvert W_i \bigg]
& = \E\left[Y_i(1) \bigvert W_i \right] \cdot \E\bigg[\frac{X_i}{\Pr(X_i = 1 \vert W_i)} \biggvert W_i \bigg] \\
& = \E\left[Y_i(1) \bigvert W_i \right] \cdot \frac{\E[X_i \vert W_i]}{\Pr(X_i = 1 \vert W_i)} \\
& = \E\left[Y_i(1) \bigvert W_i \right] \cdot \frac{\Pr(X_i = 1 \vert W_i)}{\Pr(X_i = 1 \vert W_i)} \\
& = \E\left[Y_i(1) \bigvert W_i \right].
\end{align*}
Thus, 
$$
\E\bigg[\frac{Y_i X_i}{\pi(W_i)} \biggvert W_i \bigg] = \E\left[Y_i(1) \bigvert W_i \right].
$$
So by the Law of Iterated Expectations,
$$
\mu_1 = \E\big[Y_i(1)\big] = \E\Big[\E\left[Y_i(1) \bigvert W_i\right]\Big] = $$
$$\E\Bigg[\E\bigg[\frac{Y_i X_i}{\pi(W_i)} \biggvert W_i \bigg]\Bigg] = \E\bigg[\frac{Y_i X_i}{\pi(W_i)}\bigg].
$$

The second term ($-\E \left[\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)}\right]$) obeys the same logic.  Since $\hat\beta_i$ is selected with a sample splitting procedure, we have $\hat \beta_i \independent X_i | W_i$:
\begin{align*}
\E \left[-\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)} \biggvert W_i \right] & = -\E \left[g(W_i, \hat \beta_i) \biggvert W_i \right] \E \left[\frac{ X_i}{\pi_i(W_i)} \biggvert W_i \right] \\
& = -\E[g(W_i,\hat \beta_i) | W_i].
\end{align*}
Applying the law of iterated expectations, we have $$
\E \left[-\frac{g(W_i, \hat \beta_i)X_i}{\pi_i(W_i)} \biggvert W_i \right] = -\E[g(W_i,\hat \beta_i)]
$$
which cancels with the third term ($\E[g(W_i,\hat \beta_i)]$), leaving:
$ \E[ \hat \mu_{1,R}] = \mu_1.$
\end{proof}













==> xwtjpfhppcxfqdxsdjcpxzfggcqhvbdm/stddef.tex <==
%&tex
%! TEX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%
% Brackets and functions
%%%%%%%%%%%%%%%%%%%%%%%

\DeclarePairedDelimiter\paren\lparen\rparen
\DeclarePairedDelimiter\bracket\lbrack\rbrack
\DeclarePairedDelimiter\braces\lbrace\rbrace

\DeclarePairedDelimiter\abs\lvert\rvert
\DeclarePairedDelimiter\floor\lfloor\rfloor
\DeclarePairedDelimiter\ceil\lceil\rceil

\providecommand{\bbone}{\mathbf{1}}
\DeclarePairedDelimiterXPP\indicator[1]{\bbone}{\lbrack}{\rbrack}{}{#1}

\DeclarePairedDelimiterXPP\expf[1]{\exp}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP\logf[1]{\log}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP\maxf[1]{\max}{\lparen}{\rparen}{}{#1}
\DeclarePairedDelimiterXPP\minf[1]{\min}{\lparen}{\rparen}{}{#1}

\DeclarePairedDelimiterXPP\func[2]{#1}{\lparen}{\rparen}{}{#2}


%%%%%%%%%%%%%%%%%%%%%%%
% Sets
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\set}[1]{#1}

\newcommand\suchthat{:\allowbreak\mathopen{}}
\DeclarePairedDelimiter\setb\lbrace\rbrace

\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Integers}{\mathbb{Z}}
\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\bset}{\setb{0, 1}}
\newcommand{\IntsTo}[1]{\setb{1, 2, \dotsc, #1}}
%\newcommand{\IntsTo}[1]{\bracket{#1}}
\newcommand{\IntsTon}{\IntsTo{n}}

\newcommand{\comp}{\mathsf{c}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclarePairedDelimiter\card\lvert\rvert


%%%%%%%%%%%%%%%%%%%%%%%
% Vectors and matrices
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\mat}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}

\newcommand{\arbvec}{\vec{v}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\zerovec}{\vec{0}}

\newcommand{\unitM}{\mat{I}}

\newcommand{\eigvec}[1]{\vec{\eta}_{#1}}
\newcommand{\eigval}[1]{\lambda_{#1}}
\newcommand{\eigveci}{\eigvec{i}}
\newcommand{\eigvali}{\eigval{i}}
\newcommand{\eigvalmin}{\eigval{\min}}
\newcommand{\eigvalmax}{\eigval{\max}}
\newcommand{\eigvecM}{\mat{Q}}
\newcommand{\eigvalM}{\mat{\Lambda}}

\newcommand{\basisv}[1]{\vec{e}_{#1}}

\newcommand{\inv}{{-1}}
\newcommand{\pinv}{\dagger}

% http://tex.stackexchange.com/a/217624/100722
\makeatletter
\newcommand*{\tran}{{\mathpalette\@tran{}}}
\newcommand*{\@tran}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
\makeatother

% Alternative transpose
% \newcommand{\tran}{{\mkern-1.5mu\mathsf{T}}}

\DeclarePairedDelimiter\iprod\langle\rangle

\DeclarePairedDelimiter\norm\lVert\rVert
\DeclarePairedDelimiterXPP\tnorm[1]{}{\lVert}{\rVert_{1}}{}{#1}
\DeclarePairedDelimiterXPP\enorm[1]{}{\lVert}{\rVert_{2}}{}{#1}
\DeclarePairedDelimiterXPP\inorm[1]{}{\lVert}{\rVert_{\infty}}{}{#1}
\DeclarePairedDelimiterXPP\pnorm[2]{}{\lVert}{\rVert_{#1}}{}{#2}

\DeclarePairedDelimiterXPP\detf[1]{\det}{\lparen}{\rparen}{}{#1}

\DeclareMathOperator{\trsym}{tr}
\DeclarePairedDelimiterXPP\tr[1]{\trsym}{\lparen}{\rparen}{}{#1}

\DeclareMathOperator{\diagsym}{diag}
\DeclarePairedDelimiterXPP\diag[1]{\diagsym}{\lparen}{\rparen}{}{#1}

\DeclareMathOperator{\ranksym}{rank}
\DeclarePairedDelimiterXPP\rank[1]{\ranksym}{\lparen}{\rparen}{}{#1}

\DeclareMathOperator{\vectorizesym}{vec}
\DeclarePairedDelimiterXPP\vectorize[1]{\vectorizesym}{\lparen}{\rparen}{}{#1}

%%%%%%%%%%%%%%%%%%%%%%%
% Probability
%%%%%%%%%%%%%%%%%%%%%%%

\providecommand\given{}
\newcommand\givensymbol[1]{\nonscript\:#1\vert\allowbreak\nonscript\:\mathopen{}}

\let\Prsym\Pr
\let\Pr\relax
\DeclarePairedDelimiterXPP\Pr[1]{\Prsym}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#1}

\DeclarePairedDelimiterXPP\Prsub[2]{\Prsym_{#1}}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#2}

\DeclareMathOperator{\Esym}{E}


\DeclarePairedDelimiterXPP\Esub[2]{\Esym_{#1}}{\lbrack}{\rbrack}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#2}

\DeclareMathOperator{\Varsym}{Var}
\DeclarePairedDelimiterXPP\Var[1]{\Varsym}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#1}

\DeclarePairedDelimiterXPP\Varsub[2]{\Varsym_{#1}}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#2}

\DeclarePairedDelimiterXPP\EstVar[1]{\widehat{\Varsym}}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#1}

\DeclareMathOperator{\Covsym}{Cov}
\DeclarePairedDelimiterXPP\Cov[1]{\Covsym}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#1}

\DeclarePairedDelimiterXPP\Covsub[2]{\Covsym_{#1}}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#2}

\DeclareMathOperator{\Corrsym}{Corr}
\DeclarePairedDelimiterXPP\Corr[1]{\Corrsym}{\lparen}{\rparen}{}{%
	\renewcommand\given{\givensymbol{\delimsize}}%
	#1}

% http://jblevins.org/log/latex-tips
\makeatletter
\newcommand{\indep}{\protect\mathpalette{\protect\@indep}{\perp}}
\newcommand*{\@indep}[2]{\mathrel{\rlap{$#1#2$}\mkern3mu{#1#2}}}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%
% Asymptotics
%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator*{\plim}{plim}

\newcommand{\asarrow}{\overset{a.s.}{\longrightarrow}}
\newcommand{\darrow}{\overset{d}{\longrightarrow}}
\newcommand{\parrow}{\overset{p}{\longrightarrow}}

\newcommand{\bigOsym}{\mathcal{O}}
\DeclarePairedDelimiterXPP\bigO[1]{\bigOsym}{\lparen}{\rparen}{}{#1}

\newcommand{\littleOsym}{o}
\DeclarePairedDelimiterXPP\littleO[1]{\littleOsym}{\lparen}{\rparen}{}{#1}

\newcommand{\bigOpsym}{\bigOsym_p}
\DeclarePairedDelimiterXPP\bigOp[1]{\bigOpsym}{\lparen}{\rparen}{}{#1}

\newcommand{\littleOpsym}{\littleOsym_p}
\DeclarePairedDelimiterXPP\littleOp[1]{\littleOpsym}{\lparen}{\rparen}{}{#1}

\newcommand{\bigOmegasym}{\Omega}
\DeclarePairedDelimiterXPP\bigOmega[1]{\bigOmegasym}{\lparen}{\rparen}{}{#1}

\newcommand{\littleOmegasym}{\omega}
\DeclarePairedDelimiterXPP\littleOmega[1]{\littleOmegasym}{\lparen}{\rparen}{}{#1}

\newcommand{\bigThetasym}{\Theta}
\DeclarePairedDelimiterXPP\bigTheta[1]{\bigThetasym}{\lparen}{\rparen}{}{#1}


%%%%%%%%%%%%%%%%%%%%%%%
% Misc
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\diff}{\mathop{}\!\mathrm{d}}


%%%%%%%%%%%%%%%%%%%%%%%
% Convenience macros
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\sumjn}{\sum_{j=1}^n}

\newcommand{\quadtext}[1]{\quad\text{#1}\quad}
\newcommand{\qquadtext}[1]{\qquad\text{#1}\qquad}

\newcommand{\quadand}{\quadtext{and}}
\newcommand{\qquadand}{\qquadtext{and}}

\newcommand{\quadwhere}{\quadtext{where}}
\newcommand{\qquadwhere}{\qquadtext{where}}


%%%%%%%%%%%%%%%%%%%%%%%
% Theorems etc
%%%%%%%%%%%%%%%%%%%%%%%

% Propositions in main text
\theoremstyle{plain}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}

% Referenced propositions
\newtheorem{innerrefconjecture}{Conjecture}
\newenvironment{refconjecture}[1]
{\renewcommand\theinnerrefconjecture{#1}\innerrefconjecture}
{\endinnerrefconjecture}

\newtheorem{innerrefcorollary}{Corollary}
\newenvironment{refcorollary}[1]
{\renewcommand\theinnerrefcorollary{#1}\innerrefcorollary}
{\endinnerrefcorollary}

\newtheorem{innerreflemma}{Lemma}
\newenvironment{reflemma}[1]
{\renewcommand\theinnerreflemma{#1}\innerreflemma}
{\endinnerreflemma}

\newtheorem{innerrefproposition}{Proposition}
\newenvironment{refproposition}[1]
{\renewcommand\theinnerrefproposition{#1}\innerrefproposition}
{\endinnerrefproposition}

\newtheorem{innerreftheorem}{Theorem}
\newenvironment{reftheorem}[1]
{\renewcommand\theinnerreftheorem{#1}\innerreftheorem}
{\endinnerreftheorem}

% Definitions and assumptions
\theoremstyle{definition}
\newtheorem{assumption}{Assumption}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}

% Remarks and examples
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}


%%%%%%%%%%%%%%%%%%%%%%%
% Supplement logistics
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\resetsuppcounters{%
\setcounter{section}{0}%
\setcounter{table}{0}%
\setcounter{figure}{0}%
\setcounter{equation}{0}%
\setcounter{conjecture}{0}%
\setcounter{corollary}{0}%
\setcounter{lemma}{0}%
\setcounter{proposition}{0}%
\setcounter{theorem}{0}%
\setcounter{assumption}{0}%
\setcounter{condition}{0}%
\setcounter{definition}{0}%
\setcounter{remark}{0}%
\setcounter{example}{0}%
}

\newcommand\updatesuppcounters[1]{%
\renewcommand\thesection{#1\arabic{section}}%
\renewcommand\thetable{#1\arabic{table}}%
\renewcommand\thefigure{#1\arabic{figure}}%
\renewcommand\theequation{#1\arabic{equation}}%
\renewcommand\theconjecture{#1\arabic{conjecture}}%
\renewcommand\thecorollary{#1\arabic{corollary}}%
\renewcommand\thelemma{#1\arabic{lemma}}
\renewcommand\theproposition{#1\arabic{proposition}}
\renewcommand\thetheorem{#1\arabic{theorem}}
\renewcommand\theassumption{#1\arabic{assumption}}
\renewcommand\thecondition{#1\arabic{condition}}
\renewcommand\thedefinition{#1\arabic{definition}}
\renewcommand\theremark{#1\arabic{remark}}
\renewcommand\theexample{#1\arabic{example}}
}

\newcommand\updatesuppanchors[1]{
\renewcommand\theHsection{#1.\arabic{section}}
\renewcommand\theHtable{#1.\arabic{table}}
\renewcommand\theHfigure{#1.\arabic{figure}}
\renewcommand\theHequation{#1.\arabic{equation}}
\renewcommand\theHconjecture{#1.\arabic{conjecture}}
\renewcommand\theHcorollary{#1.\arabic{corollary}}
\renewcommand\theHlemma{#1.\arabic{lemma}}
\renewcommand\theHproposition{#1.\arabic{proposition}}
\renewcommand\theHtheorem{#1.\arabic{theorem}}
\renewcommand\theHassumption{#1.\arabic{assumption}}
\renewcommand\theHcondition{#1.\arabic{condition}}
\renewcommand\theHdefinition{#1.\arabic{definition}}
\renewcommand\theHremark{#1.\arabic{remark}}
\renewcommand\theHexample{#1.\arabic{example}}
}


